Beyond the periodic orbit theory

The global constraints on chaotic dynamics induced by the analyticity of smooth flows are used to dispense with individual periodic orbits and derive infinite families of exact sum rules for several simple dynamical systems. The associated Fredholm determinants are of particularly simple polynomial form. The theory developed suggests an alternative to the conventional periodic orbit theory approach to determining eigenspectra of transfer operators.

==> xfig/f_farey_sum <==
#FIG 3.1
Portrait
Center
Inches
1200 2
6 224 1724 749 2324
4 0 -1 0 0 29 30 0.0000000 4 315 465 225 2100 F :\001
4 0 -1 0 0 0 20 0.0000000 4 195 135 434 2265 1\001
-6
6 5926 526 6301 1201
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 5928 843 6228 843
4 0 -1 0 0 0 22 0.0000000 4 210 150 6003 753 1\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 6003 1128 2\001
-6
6 1200 75 1575 750
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 1202 392 1502 392
4 0 -1 0 0 0 22 0.0000000 4 210 150 1277 677 1\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 1277 302 0\001
-6
6 10500 75 10875 750
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 10501 391 10801 391
4 0 -1 0 0 0 22 0.0000000 4 210 150 10576 301 1\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 10576 676 1\001
-6
1 3 0 1 -1 -1 0 0 -1 0.0000000 1 0.000 2776 5536 45 45 2776 5536 2776 5491
1 3 0 1 -1 -1 0 0 -1 0.0000000 1 0.000 3361 5551 45 45 3361 5551 3361 5506
1 3 0 1 -1 -1 0 0 -1 0.0000000 1 0.000 3976 5536 45 45 3976 5536 3976 5491
1 3 0 1 -1 -1 0 0 -1 0.0000000 1 0.000 4561 5551 45 45 4561 5551 4561 5506
1 3 0 1 -1 -1 0 0 -1 0.0000000 1 0.000 5761 5536 45 45 5761 5536 5761 5491
1 3 0 1 -1 -1 0 0 -1 0.0000000 1 0.000 5176 5521 45 45 5176 5521 5176 5476
1 3 0 1 -1 -1 0 0 -1 0.0000000 1 0.000 9376 5536 45 45 9376 5536 9376 5491
1 3 0 1 -1 -1 0 0 -1 0.0000000 1 0.000 6976 5551 45 45 6976 5551 6976 5506
1 3 0 1 -1 -1 0 0 -1 0.0000000 1 0.000 6346 5521 45 45 6346 5521 6346 5476
1 3 0 1 -1 -1 0 0 -1 0.0000000 1 0.000 8146 5521 45 45 8146 5521 8146 5476
1 3 0 1 -1 -1 0 0 -1 0.0000000 1 0.000 2161 5536 45 45 2161 5536 2161 5491
1 3 0 1 -1 -1 0 0 -1 0.0000000 1 0.000 9976 5536 45 45 9976 5536 9976 5491
1 3 0 1 -1 -1 0 0 -1 0.0000000 1 0.000 8776 5551 45 45 8776 5551 8776 5506
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 3526 2101 2701 2851
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 2326 3376 1951 3976
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 1651 4651 1576 5026
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 5026 3451 5326 3976
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 5776 5506 5551 4651
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 7126 3451 6826 4051
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 6601 4651 6346 5506
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 8701 2101 9526 2926
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 8926 4651 8776 5506
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 8026 4651 8146 5506
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 8326 2101 7426 2926
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 9526 3451 9151 4051
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 10201 4651 9976 5521
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 9151 4651 9376 5521
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 7801 4651 7651 5101
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 3901 2101 4651 2776
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 5326 4651 5176 5491
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 2626 3376 3001 3901
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 2926 4651 2791 5521
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 1951 4651 2161 5521
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 5851 976 3901 1726
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 6301 976 8251 1726
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 6826 4651 6961 5551
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 4726 3451 4351 4126
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 4351 4651 4546 5506
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 4126 4651 3976 5506
2 1 0 1 -1 -1 0 0 -1 0.000 0 0 -1 0 0 2
	 7426 3451 7801 3976
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 3527 1892 3827 1892
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 2327 3092 2627 3092
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 4727 3092 5027 3092
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 7127 3092 7427 3092
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 9527 3092 9827 3092
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 3226 4651 3361 5506
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 9826 3451 10126 4051
2 1 2 1 -1 -1 0 0 -1 3.000 0 0 -1 0 0 2
	 10426 4651 10501 5101
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 1652 4292 1952 4292
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 2927 4292 3227 4292
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 5252 4292 5552 4292
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 6527 4292 6827 4292
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 7727 4292 8027 4292
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 8852 4292 9152 4292
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 10127 4292 10427 4292
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 1427 5417 1727 5417
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 7427 5492 7727 5492
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 10427 5492 10727 5492
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 4052 4292 4352 4292
2 1 0 2 -1 7 0 0 -1 0.000 0 0 -1 0 0 2
	 8327 1892 8627 1892
4 0 -1 0 0 29 30 0.0000000 4 315 465 226 1051 F :\001
4 0 -1 0 0 29 30 0.0000000 4 315 465 226 3226 F :\001
4 0 -1 0 0 29 30 0.0000000 4 315 465 226 4351 F :\001
4 0 -1 0 0 29 30 0.0000000 4 315 465 226 5551 F :\001
4 0 -1 0 0 0 20 0.0000000 4 195 135 435 1216 0\001
4 0 -1 0 0 0 20 0.0000000 4 195 135 435 3391 2\001
4 0 -1 0 0 0 20 0.0000000 4 195 135 435 4516 3\001
4 0 -1 0 0 0 20 0.0000000 4 195 135 435 5716 4\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 3602 1802 1\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 2402 3002 1\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 3602 2177 3\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 2402 3377 4\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 8402 1802 2\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 8402 2177 3\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 4802 3002 2\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 4802 3377 5\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 7202 3002 3\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 7202 3377 5\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 9602 3002 3\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 9602 3377 4\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 1727 4202 1\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 1502 5327 1\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 1727 4577 5\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 1502 5702 6\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 3002 4202 2\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 3002 4577 7\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 4127 4202 3\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 4127 4577 8\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 5327 4202 3\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 5327 4577 7\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 6602 4577 7\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 8927 4577 7\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 10202 4577 5\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 7802 4577 8\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 6602 4202 4\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 7802 4202 5\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 8927 4202 5\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 10202 4202 4\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 10502 5402 5\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 10502 5777 6\001
4 0 -1 0 0 0 22 0.0000000 4 210 300 7502 5777 13\001
4 0 -1 0 0 0 22 0.0000000 4 210 150 7502 5402 8\001

